Chickenpox Cases in Hungary: a Benchmark Dataset for Spatiotemporal Signal Processing with Graph Neural Networks

Recurrent graph convolutional neural networks are highly effective machine learning techniques for spatiotemporal signal processing. Newly proposed graph neural network architectures are repetitively evaluated on standard tasks such as traffic or weather forecasting. In this paper, we propose the Chickenpox Cases in Hungary dataset as a new dataset for comparing graph neural network architectures. Our time series analysis and forecasting experiments demonstrate that the Chickenpox Cases in Hungary dataset is adequate for comparing the predictive performance and forecasting capabilities of novel recurrent graph neural network architectures.

==> plots/correlation.tex <==
\begin{figure}
\begin{tikzpicture}
	\tikzset{font={\fontsize{7pt}{12}\selectfont}}
\begin{axis}[
    axis equal image, % We want a square grid, not a rectangular one
    scatter, % This activates the color mapping
    colormap/viridis, % Choose the colormap
    colorbar, % Add a legend
    point meta min=-1,
    point meta max=1,
    ytick={0,1,2,3,4,5,6,7,8,9,10,11,12,13,14,15,16,17,18,19},
    yticklabels={Bacs,Baranya,Bekes,Borsod,Budapest,Csongrad,Fejer,Gyor,Hajdu,Heves,Jasz,Komarom,Nograd,Pest,Somogy,Szabolcs,Tolna,Vas,Veszprem,Zala},
    xticklabels={,,}.
    grid=minor, % Grid lines between the intervals
    minor tick num=1, % One minor tick per interval
    tickwidth=0pt, % Don't draw the major tick marks
    y dir=reverse, % Y increases downward
    xticklabel pos=right, % X axis labels go to the top
    enlargelimits={abs=0.5}, % Add half a unit on all sides
    scatter/@pre marker code/.append code={% A bit of magic for scaling the circles in axis units
      \pgfplotstransformcoordinatex{sqrt(abs(\pgfplotspointmeta))}% Area scales with the square of the radius
      \scope[mark size=\pgfplotsunitxlength*\pgfmathresult/2, fill=mapped color]
    },
    scatter/@post marker code/.append code={%
      \endscope%
    }
]
\addplot +[
    point meta=explicit, % We'll provide values for the color and size
    only marks, % No lines between the points
    ] table [
    x expr={int(mod(\coordindex+0.01,20))}, % The position depends on the coordinate index, not the X or Y values
    y expr={int((\coordindex+0.01)/20))},
    meta=value
] {
X   Y   value

0 0 1.0
0 1 0.0511
0 2 0.1011
0 3 0.1089
0 4 0.2789
0 5 0.1037
0 6 0.1778
0 7 0.2655
0 8 0.0814
0 9 0.2357
0 10 0.2331
0 11 0.2019
0 12 0.2736
0 13 0.2023
0 14 0.1716
0 15 0.1336
0 16 0.0148
0 17 0.1146
0 18 -0.0099
0 19 -0.1031
1 0 0.0511
1 1 1.0
1 2 0.0761
1 3 0.169
1 4 0.2035
1 5 0.2039
1 6 0.2047
1 7 0.1188
1 8 0.1138
1 9 0.2466
1 10 0.2084
1 11 0.1042
1 12 0.1965
1 13 0.2799
1 14 0.3064
1 15 0.162
1 16 0.116
1 17 0.1615
1 18 0.2253
1 19 0.1219
2 0 0.1011
2 1 0.0761
2 2 1.0
2 3 0.1751
2 4 0.2692
2 5 0.0876
2 6 0.1425
2 7 0.1386
2 8 0.0828
2 9 0.1123
2 10 0.2495
2 11 0.1843
2 12 0.0465
2 13 0.1833
2 14 0.0891
2 15 -0.083
2 16 0.026
2 17 0.1872
2 18 0.0981
2 19 0.1315
3 0 0.1089
3 1 0.169
3 2 0.1751
3 3 1.0
3 4 0.3307
3 5 0.1657
3 6 0.1889
3 7 0.0456
3 8 0.2382
3 9 0.1114
3 10 0.192
3 11 0.1072
3 12 0.0833
3 13 0.2287
3 14 0.1862
3 15 0.221
3 16 0.1063
3 17 0.1669
3 18 0.1429
3 19 0.0786
4 0 0.2789
4 1 0.2035
4 2 0.2692
4 3 0.3307
4 4 1.0
4 5 0.2944
4 6 0.1847
4 7 0.2747
4 8 0.3036
4 9 0.343
4 10 0.2224
4 11 0.3197
4 12 0.3281
4 13 0.4053
4 14 0.301
4 15 0.0892
4 16 0.2216
4 17 0.2483
4 18 0.238
4 19 0.1194
5 0 0.1037
5 1 0.2039
5 2 0.0876
5 3 0.1657
5 4 0.2944
5 5 1.0
5 6 0.3002
5 7 0.16
5 8 0.1277
5 9 0.265
5 10 0.0818
5 11 0.0572
5 12 0.2905
5 13 0.1389
5 14 0.1642
5 15 -0.0037
5 16 0.075
5 17 0.1845
5 18 0.2574
5 19 0.105
6 0 0.1778
6 1 0.2047
6 2 0.1425
6 3 0.1889
6 4 0.1847
6 5 0.3002
6 6 1.0
6 7 0.2562
6 8 0.2466
6 9 0.3084
6 10 0.296
6 11 0.0224
6 12 0.215
6 13 0.1798
6 14 0.1864
6 15 0.1238
6 16 0.1447
6 17 0.2214
6 18 0.2445
6 19 0.1432
7 0 0.2655
7 1 0.1188
7 2 0.1386
7 3 0.0456
7 4 0.2747
7 5 0.16
7 6 0.2562
7 7 1.0
7 8 0.253
7 9 0.1736
7 10 0.2794
7 11 0.2881
7 12 0.3255
7 13 0.3141
7 14 0.1331
7 15 0.1055
7 16 0.0928
7 17 0.2371
7 18 0.2541
7 19 0.011
8 0 0.0814
8 1 0.1138
8 2 0.0828
8 3 0.2382
8 4 0.3036
8 5 0.1277
8 6 0.2466
8 7 0.253
8 8 1.0
8 9 0.2413
8 10 0.2167
8 11 0.2567
8 12 0.1214
8 13 0.303
8 14 0.1958
8 15 0.1787
8 16 0.096
8 17 0.1414
8 18 0.3065
8 19 0.0747
9 0 0.2357
9 1 0.2466
9 2 0.1123
9 3 0.1114
9 4 0.343
9 5 0.265
9 6 0.3084
9 7 0.1736
9 8 0.2413
9 9 1.0
9 10 0.2566
9 11 0.1511
9 12 0.3095
9 13 0.4102
9 14 0.253
9 15 0.1966
9 16 0.1418
9 17 0.1552
9 18 0.2252
9 19 0.1128
10 0 0.2331
10 1 0.2084
10 2 0.2495
10 3 0.192
10 4 0.2224
10 5 0.0818
10 6 0.296
10 7 0.2794
10 8 0.2167
10 9 0.2566
10 10 1.0
10 11 0.1794
10 12 0.171
10 13 0.1987
10 14 0.0975
10 15 0.1781
10 16 0.0972
10 17 0.2362
10 18 0.2648
10 19 0.1483
11 0 0.2019
11 1 0.1042
11 2 0.1843
11 3 0.1072
11 4 0.3197
11 5 0.0572
11 6 0.0224
11 7 0.2881
11 8 0.2567
11 9 0.1511
11 10 0.1794
11 11 1.0
11 12 0.1234
11 13 0.3291
11 14 0.1915
11 15 0.1538
11 16 0.016
11 17 0.2048
11 18 0.1018
11 19 0.1483
12 0 0.2736
12 1 0.1965
12 2 0.0465
12 3 0.0833
12 4 0.3281
12 5 0.2905
12 6 0.215
12 7 0.3255
12 8 0.1214
12 9 0.3095
12 10 0.171
12 11 0.1234
12 12 1.0
12 13 0.2923
12 14 0.1553
12 15 0.0988
12 16 0.1901
12 17 0.1346
12 18 0.1552
12 19 0.2186
13 0 0.2023
13 1 0.2799
13 2 0.1833
13 3 0.2287
13 4 0.4053
13 5 0.1389
13 6 0.1798
13 7 0.3141
13 8 0.303
13 9 0.4102
13 10 0.1987
13 11 0.3291
13 12 0.2923
13 13 1.0
13 14 0.3051
13 15 0.3195
13 16 0.2197
13 17 0.248
13 18 0.2779
13 19 0.0977
14 0 0.1716
14 1 0.3064
14 2 0.0891
14 3 0.1862
14 4 0.301
14 5 0.1642
14 6 0.1864
14 7 0.1331
14 8 0.1958
14 9 0.253
14 10 0.0975
14 11 0.1915
14 12 0.1553
14 13 0.3051
14 14 1.0
14 15 0.1875
14 16 0.2008
14 17 0.1527
14 18 0.2191
14 19 0.072
15 0 0.1336
15 1 0.162
15 2 -0.083
15 3 0.221
15 4 0.0892
15 5 -0.0037
15 6 0.1238
15 7 0.1055
15 8 0.1787
15 9 0.1966
15 10 0.1781
15 11 0.1538
15 12 0.0988
15 13 0.3195
15 14 0.1875
15 15 1.0
15 16 0.1765
15 17 -0.0004
15 18 0.1129
15 19 0.0968
16 0 0.0148
16 1 0.116
16 2 0.026
16 3 0.1063
16 4 0.2216
16 5 0.075
16 6 0.1447
16 7 0.0928
16 8 0.096
16 9 0.1418
16 10 0.0972
16 11 0.016
16 12 0.1901
16 13 0.2197
16 14 0.2008
16 15 0.1765
16 16 1.0
16 17 0.1011
16 18 0.169
16 19 0.1001
17 0 0.1146
17 1 0.1615
17 2 0.1872
17 3 0.1669
17 4 0.2483
17 5 0.1845
17 6 0.2214
17 7 0.2371
17 8 0.1414
17 9 0.1552
17 10 0.2362
17 11 0.2048
17 12 0.1346
17 13 0.248
17 14 0.1527
17 15 -0.0004
17 16 0.1011
17 17 1.0
17 18 0.1943
17 19 0.136
18 0 -0.0099
18 1 0.2253
18 2 0.0981
18 3 0.1429
18 4 0.238
18 5 0.2574
18 6 0.2445
18 7 0.2541
18 8 0.3065
18 9 0.2252
18 10 0.2648
18 11 0.1018
18 12 0.1552
18 13 0.2779
18 14 0.2191
18 15 0.1129
18 16 0.169
18 17 0.1943
18 18 1.0
18 19 0.1688
19 0 -0.1031
19 1 0.1219
19 2 0.1315
19 3 0.0786
19 4 0.1194
19 5 0.105
19 6 0.1432
19 7 0.011
19 8 0.0747
19 9 0.1128
19 10 0.1483
19 11 0.1483
19 12 0.2186
19 13 0.0977
19 14 0.072
19 15 0.0968
19 16 0.1001
19 17 0.136
19 18 0.1688
19 19 1.0
};
\end{axis}
\end{tikzpicture}
\caption{Caption text}
\end{figure}
